Low-shot Object Learning with Mutual Exclusivity Bias

This paper introduces Low-shot Object Learning with Mutual Exclusivity Bias (LSME), the first computational framing of mutual exclusivity bias, a phenomenon commonly observed in infants during word learning. We provide a novel dataset, comprehensive baselines, and a state-of-the-art method to enable the ML community to tackle this challenging learning task. The goal of LSME is to analyze an RGB image of a scene containing multiple objects and correctly associate a previously-unknown object instance with a provided category label. This association is then used to perform low-shot learning to test category generalization. We provide a data generation pipeline for the LSME problem and conduct a thorough analysis of the factors that contribute to its difficulty. Additionally, we evaluate the performance of multiple baselines, including state-of-the-art foundation models. Finally, we present a baseline approach that outperforms state-of-the-art models in terms of low-shot accuracy.

==> figure_text/multi_setting.tex <==
%%%% ABC, Toys, ShapeNet datasets
\begin{wrapfigure}{l}{0.5\textwidth}

\vspace{-20pt}
\centering
\includegraphics[width=\linewidth]{figures/multi_setting.pdf}
\caption{\textbf{Left:} Synthetic data rendered from ModelNet and ABC (first and second columns) for self-supervised learning of representations and low-shot testing data from ModelNet (third column). \textbf{Right:} Real data from CO3D for self-supervised representation training and low-shot testing.}
\label{fig:shot_assignment}
\vspace{-20pt}

\end{wrapfigure}

% \caption{}
% \label{fig:setting_overview}
% \vspace{-20pt}

==> figure_text/single_setting.tex <==
%%%% ABC, Toys, ShapeNet datasets
\begin{wrapfigure}{r}{0.5\textwidth}
% \begin{figure}[t!]
\vspace{-20pt}
\centering
\includegraphics[width=\linewidth]{figures/single_setting.pdf}
\caption{\textbf{Left:} Synthetic data rendered from ModelNet and ABC (first and second columns) for self-supervised learning of representations and low-shot testing data from ModelNet (third column). \textbf{Right:} Real data from CO3D for self-supervised representation training and low-shot testing.}
\label{fig:shot_assignment}
\vspace{-20pt}
% \end{figure}
\end{wrapfigure}

% \caption{}
% \label{fig:setting_overview}
% \vspace{-20pt}

==> tables/base_ablation.tex <==
\begin{table}[t!]
\renewcommand{\arraystretch}{1.0}
\begin{center}
\caption{.}
\scalebox{0.9}{
\begin{tabular}{l|c|c|c|c}\\
Method & \multicolumn{2}{c|}{DINOv2} & \multicolumn{2}{c}{Ours-DINOv2-ABC}\\
& LSA & SA & LSA & SA\\
\hline
500 scenes &41.26\ci{1.15} &52.28\ci{1.86} & 50.37\ci{1.25}&64.64\ci{1.89} \\
500 scenes (16 views/scene) & 41.58\ci{1.16}&55.20\ci{1.89}&50.72\ci{1.25}&66.68\ci{1.86}\\
8000 scenes & 43.56\ci{1.17} &61.64\ci{1.91} &54.82\ci{1.21} &76.32\ci{1.68}

\label{tbl:shapenet-res-table}
\end{tabular}}
\end{center}
\vspace{-20pt}
\end{table}

==> tables/iou.tex <==
% \begin{table}[t!]
% \renewcommand{\arraystretch}{1.0}
% \begin{center}
% \caption{The performance of different methods under LSME setting on Toys4k with two object segmenters. The quality of the instance masks plays a significant role in the low-shot and shot assignment performance for all methods.}
% \scalebox{0.9}{
% \begin{tabular}{l|c|c|c|c|c|c|c|c}\\
% Method & \multicolumn{2}{c|}{mIoU} & \multicolumn{2}{c|}{DINOv1 S/8} & \multicolumn{2}{c}{DINOv2 S/14}&\multicolumn{2}{c}{DINOv2 B/14}\\
% & Support & Query & LSA & SA & LSA & SA & LSA & SA\\
% \hline
% FreeSOLO~\cite{wang2022freesolo} & 0.74 & 0.76 & \begin{tabular}{@{}c@{}}30.05\vspace{-2pt}\\ \ci{0.84} \end{tabular} & \begin{tabular}{@{}c@{}}38.932\vspace{-2pt}\\ \ci{1.92} \end{tabular} & \begin{tabular}{@{}c@{}}32.03\vspace{-2pt}\\ \ci{0.90} \end{tabular} & \begin{tabular}{@{}c@{}}41.72\vspace{-2pt}\\ \ci{2.01} \end{tabular} & \begin{tabular}{@{}c@{}}33.22\vspace{-2pt}\\ \ci{0.99} \end{tabular} & \begin{tabular}{@{}c@{}}44.04\vspace{-2pt}\\ \ci{1.90} \end{tabular}\\
% FreeSOLO-ABC & 0.85 & 0.86 & \begin{tabular}{@{}c@{}}36.44\vspace{-2pt}\\ \ci{1.08} \end{tabular}& \begin{tabular}{@{}c@{}}46.92 \vspace{-2pt}\\ \ci{2.04} \end{tabular}& \begin{tabular}{@{}c@{}}37.08 \vspace{-2pt}\\ \ci{1.05} \end{tabular}& \begin{tabular}{@{}c@{}}48.16 \vspace{-2pt}\\ \ci{1.87} \end{tabular}& \begin{tabular}{@{}c@{}}39.24\vspace{-2pt}\\ \ci{1.17} \end{tabular}& \begin{tabular}{@{}c@{}}50.88 \vspace{-2pt}\\ \ci{1.91} \end{tabular}

% \label{tab:iou}
% \end{tabular}}
% \end{center}
% \vspace{-20pt}
% \end{table}

\begin{table}[t!]
\renewcommand{\arraystretch}{1.0}
\begin{center}
\caption{The performance of different methods under LSME setting on Toys4k with two object segmenters. The quality of the instance masks plays a significant role in the low-shot and shot assignment performance for all methods.}
\scalebox{0.9}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
Method & \multicolumn{2}{c|}{mIoU} & \multicolumn{2}{c|}{DINOv1 S/8} & \multicolumn{2}{c}{DINOv2 S/14}&\multicolumn{2}{c}{DINOv2 B/14}\\
& Support & Query & LSA & SA & LSA & SA & LSA & SA\\
\hline
FreeSOLO~\cite{wang2022freesolo} & 0.74 & 0.76 & \begin{tabular}{@{}c@{}}30.05\vspace{-2pt} \end{tabular} & \begin{tabular}{@{}c@{}}38.93\vspace{-2pt} \end{tabular} & \begin{tabular}{@{}c@{}}32.03\vspace{-2pt} \end{tabular} & \begin{tabular}{@{}c@{}}41.72\vspace{-2pt}\end{tabular} & \begin{tabular}{@{}c@{}}33.22\vspace{-2pt}\end{tabular} & \begin{tabular}{@{}c@{}}44.04\vspace{-2pt}\end{tabular}\\
FreeSOLO-ABC & 0.85 & 0.86 & \begin{tabular}{@{}c@{}}36.44\vspace{-2pt} \end{tabular}& \begin{tabular}{@{}c@{}}46.92 \vspace{-2pt} \end{tabular}& \begin{tabular}{@{}c@{}}37.08 \vspace{-2pt} \end{tabular}& \begin{tabular}{@{}c@{}}48.16 \vspace{-2pt}\end{tabular}& \begin{tabular}{@{}c@{}}39.24\vspace{-2pt}\end{tabular}& \begin{tabular}{@{}c@{}}50.88 \vspace{-2pt} \end{tabular}

\label{tab:iou}
\end{tabular}}
\end{center}
\vspace{-20pt}
\end{table}
